Gaussian Process Bandit Optimization of the Thermodynamic Variational Objective

Achieving the full promise of the Thermodynamic Variational Objective (TVO), a recently proposed variational lower bound on the log evidence involving a one-dimensional Riemann integral approximation, requires choosing a "schedule" of sorted discretization points. This paper introduces a bespoke Gaussian process bandit optimization method for automatically choosing these points. Our approach not only automates their one-time selection, but also dynamically adapts their positions over the course of optimization, leading to improved model learning and inference. We provide theoretical guarantees that our bandit optimization converges to the regret-minimizing choice of integration points. Empirical validation of our algorithm is provided in terms of improved learning and inference in Variational Autoencoders and Sigmoid Belief Networks.

==> draw_alg.tex <==
\section{From Evidence Maximization to Regret Minimization}\label{sec:bandits}

%we will frequently refer to as $\mathcal{L}_i := \TVO(\theta_i, \phi_i, \vbeta_i, \vx)$, where subscript $i$ indexes the set of parameters $\{\theta_i, \phi_i, \vbeta_i\}$ at epoch $i \in \{0, 1, ...,T\}$. % given by Eq. (\ref{eq:left_Riemann_sum}),
We view the vector $\vbeta \in [0,1]^d$ as an arm \cite{Auer2002nonstochastic} to be pulled in a continuous space, given a fixed resource of $T$ training epochs. After each round, we receive an estimate of the log evidence $\mathcal{L}$,  from which we will construct a reward function. An important feature of our problem is that the integrand in \cref{fig:tvo} changes between rounds as training progresses. Thus, our multi-armed bandit problem is said to be \textit{time-varying}, in that the optimal arm and reward function depend on round $t$.

More formally, we define the time-varying reward function $f_{t}:[0,1]^d\rightarrow\mathbb{R}$ which takes an input $\vbeta_{t}$ and produces reward $f_{t}(\vbeta_{t})$. At each round we get access to a noisy reward ${y_t=f_{t}(\vbeta_{t})+\epsilon_t}$ where we assume Gaussian noise $\epsilon_{t}\sim\mathcal{N}(0,\sigma_{f}^{2})$.  We aim to maximize the cumulative reward $\sum_{t=1}^{T/w}f_{t}(\vbeta_{t})$ across $T/w$ rounds, where $w$ is a divisor of $T$ and will later control the ratio of bandit rounds $t$ to training epochs $i$.

%using Eq. \cref{eq:left_Riemann_sum} for example.  In practice, we use a trapezoid approximation of the integral in Eq. \cref{eq:ti_integral}, evaluated at a static uniform schedule $\vbeta_0$ with $d=50$, so that $\mathcal{L}_i := \TVO(\theta_i, \phi_i, \vbeta_0, \vx)$ at training iteration $i$.
% The reward function reflects a \gls{TVO} estimate of the model evidence.  For example, we can use Eq. \cref{eq:left_Riemann_sum}  evaluated at a static uniform schedule $\vbeta_0$ with $d=50$, so that $\mathcal{L}_t := \TVO(\theta_t, \phi_t, \vbeta_0, \vx)$ at bandit round $t$.  \rb{Really hard to work the Trapz approximation in here...} We found this approach to be useful in decoupling estimation of the reward function from the choice of $\vbeta$ used to train $\{\theta, \phi\}$.  Finally, we choose the reward function $f_t(\vbeta)$ to be the improvement in $\mathcal{L}_t$ since the last round (see Eq. \ref{eq:reward_function}).

Maximizing the cumulative reward is equivalent to minimizing the \textit{cumulative regret}
\begin{align}
    R_{T/w} := \sum_{t=1}^{T/w} f_{t}(\vbeta_t^*) - f_{t}(\vbeta_t), \label{eq:cumulative_regret}
\end{align}
where $r_t := f_{t}(\vbeta_t^*) - f_{t}(\vbeta_t)$ is the \textit{instantaneous regret} defined by the difference between the received reward $f_{t}(\vbeta_t)$ and maximum reward attainable $ f_{t}(\vbeta_t^*)$ at round $t$. The regret, which is non-negative and monotonic, is more convenient to work with than the cumulative reward and will allow us to derive upper bounds in \S \ref{sec:convergence}.

% \begin{figure*}
% \includegraphics[width=0.33\columnwidth]{fig/function_S10.pdf}
% \includegraphics[width=0.33\columnwidth]{fig/function_S50.pdf}
% \includegraphics[width=0.33\columnwidth]{fig/function_S100.pdf}
% \caption{Example of the time-varying reward functions $f_t(\bbeta_t)$ using different $S=10,50,100$. We show $100$ choices of $\beta_t$ from epochs $2000-3000$ as the dots. The high level of noise makes the gradient-based approach inappropriate.  \label{fig:exmaple_function_S}}
% \end{figure*}

In order to translate the problem of maximizing the log evidence as a function of $\vbeta$ into the bandits framework, we define a time-varying reward function $f_t(\vbeta_t)$.   We construct this reward in such a way that minimizing the cumulative regret is equivalent to maximizing the final log evidence estimate $\mathcal{L}_T := \log p_{\theta_{T}}(\vx)$, i.e., such that $\min R_{T/w} = \max \mathcal{L}_T$.
% In order to translate the problem of maximizing the log evidence as a function of $\vbeta$ into the bandits framework, we must define a time-varying reward function $f_t(\vbeta_t)$.   We construct this reward in such a way that minimizing the cumulative regret is equivalent to maximizing the final log evidence estimate $\mathcal{L}_T := \log p_{\theta_{T}}(\vx)$, i.e., such that $\min R_{T/w} = \max \mathcal{L}_T$.
% 

Such a reward function can be defined by partitioning the $T$ training epochs into windows of equal length $w$, and defining the reward for each window $t \in \{0, 1, ..., T/w - 1\}$ 
\begin{align}
    f_{t}(\vbeta_{t}):=\mathcal{L}_{w(t+1)} - \mathcal{L}_{wt}\label{eq:reward_function}
\end{align}
as the difference between the \gls{TVO} log evidence estimate one window-length in the future $\mathcal{L}_{w(t+1)}$ and the present estimate $\mathcal{L}_{wt}$. Then, the cumulative reward is given by a telescoping sum over windows 
\begin{align}
\sum_{t=0}^{T/w~-~1}f_{t}(\vbeta_{t}) &= 
\big(\mathcal{L}_{w} - \mathcal{L}_{0}\big) + 
\big(\mathcal{L}_{2w} - \mathcal{L}_{w}\big) + ... + \big(\mathcal{L}_{(T/w)w} - \mathcal{L}_{(T/w~-~1)w}\big)\\
                                  &= \mathcal{L}_T - \mathcal{L}_0, \label{eq:cumulative_reward_function}
\end{align}
where $\mathcal{L}_0$ is the initial (i.e. untrained) loss. Recalling the definition of cumulative regret in Eq. \cref{eq:cumulative_regret},
\begin{align} \label{eq:equivalent_minregret_maxTVO}
    \min R_{T/w} &= \min\left(\sum_{t=0}^{T/w~-~1}f_{t}(\vbeta_t^*)\right) - \left(\sum_{t=0}^{T/w~-~1}f_{t}(\vbeta_t)\right)\\
                 &= \min\biggl(\left(\mathcal{L}^*_T - \mathcal{L}_0\right) - \left(\mathcal{L}_T - \mathcal{L}_0\right)\biggr)  \label{eq:L_T_optimal}\\
                 &= \min~(\text{const} - \mathcal{L}_T) \\
                 &= \max\mathcal{L}_T.
\end{align}
Therefore minimizing the cumulative regret for the reward function defined by Eq. \cref{eq:reward_function} is equivalent to maximizing the log evidence on the final epoch. Next, we describe how to design an optimal decision mechanism to minimize the cumulative regret $R_{T/w}$ using Gaussian processes.

%, $d$ is the dimension of $\vbeta$

\begin{algorithm}
\caption{GP-bandit for TVO (high level)\label{alg:TVO_GPTV_highlevel}}
%\vu{the reward function $f_{t}(\vbeta_{t})$ where $\vbeta_t \in [0,1]^d$, update frequency $w$}
\begin{algor}
\item [{{*}}] Input: schedule dimension $d$, reward function $f_{t}(\vbeta_{t})$ where $\vbeta_t \in [0,1]^d$ , update frequency $w$
\end{algor}
\begin{algor}[1]
\item [{for}] $t=1....T$
\item [{{*}}] Train the TVO and get $\mathcal{L}_{t}$ from Eq. (\ref{eq:left_Riemann_sum}) given previously obtained $\vbeta_{t-1}$
\item [{if}] mod$(t,w)=0$ : time to update $\vbeta_t$
\item [{{*}}] Estimate the utility $y_{t}=\mathcal{L}_{t}-\mathcal{L}_{t-w}$ and augment
$D_{t}=D_{t-1}\cup\left(\vbeta_{t-1},t,y_{t}\right)$
\item [{{*}}] Fit a time-varying, permutation invariant GP to $D_{t}$ 
\item [{{*}}] Estimate $\mu_{t}(\vbeta),\sigma_{t}(\vbeta)$ from Eqs.
(\ref{eq:GP_mean},\ref{eq:GP_var}) 
\item [{{*}}] Select $\vbeta_{t}=\arg\max \mu_{t}(\vbeta)+\sqrt{\kappa_{t}}\sigma_{t}(\vbeta)$ where $\kappa_{t}$ is from Theorem \ref{thm:theorem_sublinear_regret}
\item [{endif}]~
\item [{endfor}]~
\end{algor}
\end{algorithm}
\section{Minimizing Regret with Gaussian Processes}\label{sec:gp}
There are two unresolved problems with the reward function defined in Eq. (\ref{eq:reward_function}) which still must be addressed. The first is that it is not in fact computable, due to its use of future observations. The second is that it ignores the ordering constraint required for $\vbeta$ to be a valid Riemann partition.

We can handle both by problems by using a permutation-invariant Gaussian process to form a surrogate for the reward function $f_{t}(\vbeta_{t})$. The surrogate model will be updated by past rewards, and used in place of $f_{t}(\vbeta_{t})$ to select the next schedule at the current round, as described in Algorithm \ref{alg:TVO_GPTV_highlevel}.



In \S \ref{sec:TVGP} we formally define how to use (time-varying) Gaussian processes in bandit optimization, before describing how our permutation-invariant kernel can be used to solve the problem of ordering constraints on $\vbeta$ in \S \ref{sec:perm_invar}. Finally in \S \ref{sec:convergence} we provide a theoretical guarantee that our bandit optimization will converge to the regret-minimizing choice of  $\vbeta$. %derive the convergence analysis , which 
% theoretical guarantees that our bandit optimization converges to the regret-minimizing choice of integration points

\subsection{Time-varying Gaussian processes for Bandit Optimization} \label{sec:TVGP}
A popular design   in handling time-varying functions \cite{Krause_2011Contextual,Swersky_2013Multi,klein2017fast,nyikosa2018adaptive} such as $f_{t}(\vbeta_{t})$ is to jointly model the spatial and temporal dimensions using a product of covariance functions ${k=k_{\beta}\otimes k_{T}}$, where ${k_{\beta}:[0, 1]^d\times [0, 1]^d\rightarrow\mathbb{R}}$ is a spatial covariance function over actions, ${k_{T}:\mathbb{N}\times\mathbb{N}\rightarrow\mathbb{R}}$ is a temporal covariance function, and ${k:\mathbb{R}_+^{d+1}\times\mathbb{R}_+^{d+1}\rightarrow\mathbb{R}}$.

Under this joint modeling framework, the GP is defined as follows. At round $t$ we have the history of rewards $\bm{y}_t = [y_0, ..., y_t]^T$ and sample points $\bm{X}_t = \{\bm{x}_0, ..., \bm{x}_t\}$, where we define $\bm{x}_t \in \mathbb{R}^{d+1}$ to be the concatenation of $\vbeta_t$ and timestep $t$, i.e $\bm{x}_t:= [\vbeta_t, t]^T$. Then the time-varying reward function is GP-distributed according to
\begin{align}
    f_t \sim GP\bigl(0, k(\bm{x}, \bm{x}')\bigr) \quad \quad \quad
    \text{where } k(\bm{x}, \bm{x}') := k_{\beta}(\vbeta, \vbeta') \times k_{T}(t, t'),
\end{align}
where we have assumed zero prior mean for simplicity. For theoretical convenience we follow \cite{bogunovic2016time} and choose ${k_{T}(t,t')=(1-\omega)^{\frac{|t-t'|}{2}}}$, where $\omega$ is a ``forgetting-remembering'' trade-off parameter learned from data. We describe $k_{\beta}(\vbeta, \vbeta')$ in \S \ref{sec:perm_invar}.

Using standard Gaussian identities \cite{Bishop_2006pattern,Rasmussen_2006gaussian}, the posterior predictive is also GP distributed, with mean and variance given by
\begin{align}
\mu_t(\vbeta_*) &= \bm{k}_t(\vbeta_*)^T\left(\bm{K}_t + \sigma_{f}^{2}\bm{I} \right)^{-1}\bm{y}_t \label{eq:GP_mean} \\
\sigma_t^2(\vbeta_*) &= \bm{k}_t(\vbeta_*, \vbeta_*) - \bm{k}_t(\vbeta_*)^T\left(\bm{K}_t + \sigma_{f}^{2}\bm{I} \right)^{-1}\bm{k}_t(\vbeta_*)\label{eq:GP_var}
\end{align}
where $\bm{k}_t(\vbeta) = [k(\bm{x}_0, \bm{x}), ... , k(\bm{x}_t, \bm{x})]^T$ and $\bm{K}_t = [k(\bm{x}, \bm{x}')]_{\bm{x}, \bm{x}' \in \bm{X}_t}$. Using this permutation-invariant, time-varying GP we can select $\vbeta_{t+1}$ by maximizing a linear combination of the GP posterior mean and variance w.r.t $\vbeta_t$
\begin{align}
\vbeta_{t+1}&= \argmax_{\vbeta_t}\mu_t(\vbeta_t) + \sqrt{\kappa_{t}}\sigma_t(\vbeta_t),
\label{eq:acquisition_function}
\end{align}
where Eq. (\ref{eq:acquisition_function}) is referred to as an \textit{acquisition function} and $\kappa_{t}$ is its exploration-exploitation trade-off parameter. We note that there are other acquisition functions available \cite{Jones_1998Efficient,Hennig_2012Entropy,Hernandez_2014Predictive}. Our acquisition function, Eq. (\ref{eq:acquisition_function}), is the time-varying version of GP-UCB \cite{Srinivas_2010Gaussian,bogunovic2016time}, which allows us to obtain convergence results in \S\ref{sec:convergence} and set $\kappa_{t}$ in Theorem \ref{thm:theorem_sublinear_regret}. 

% The acquisition function can be optimized using any standard optimization toolkit~\cite{fletcher2013practical,Jones_1993Lipschitzian}.

% \subsection{Permutation Invariant Spacial Kernel}\label{sec:perm_invar}
\subsection{Ordering Constraints and Permutation Invariance}\label{sec:perm_invar}
% \vm{Vu I'm being intentionally cautious here - we can add more arguments to this section after  submission. Frank wrote the below discussion. }


% \begin{algorithm}
% \caption{TVO-GPTV (high level)\label{alg:TVO_GPTV_highlevel}}

% \begin{algor}
% \item [{{*}}] Input: the reward function $f_{t}(\vbeta_{t})$, $d$ is
% dimension of $\vbeta$, update frequency $w$
% \end{algor}
% \begin{algor}[1]
% \item [{for}] $t=1....T$
% \item [{{*}}] Train the TVO objective function given $\vbeta_{t-1}$ obtained
% previously
% \item [{if}] mod$(t,w)=0$ : time to update $\vbeta_t$
% \item [{{*}}] Estimate the utility $y_{t}=\mathcal{L}_{t}-\mathcal{L}_{t-w}$ and augment
% $D_{t}=D_{t-1}\cup\left(\vbeta_{t-1},t,y_{t}\right)$
% \item [{{*}}] Fit a time-varying, permutation invariant GP to $D_{t}$ 
% \item [{{*}}] Estimate $\mu_{t}(\vbeta),\sigma_{t}(\vbeta)$ from Eqs.
% (\ref{eq:GP_mean},\ref{eq:GP_var}) 
% \item [{{*}}] Select $\vbeta_{t}=\arg\max \mu_{t}(\vbeta)+\sqrt{\kappa_{t}}\sigma_{t}(\vbeta)$ where $\kappa_{t}$ is from Theorem \ref{thm:theorem_sublinear_regret}
% \item [{endif}]~
% \item [{endfor}]~
% \end{algor}
% \end{algorithm}



Recall that the vector $\vbeta=\left[\beta_{0},...,\beta_{d-1}\right]^T$ holds the locations of the left Riemann integral approximation in Eq. \eqref{eq:left_Riemann_sum}. In order for the left Riemann approximation to the \gls{TVO} to be sensible, there must be an ordering constraint imposed on $\bbeta$ such that $0 < \beta_1 < ... < \beta_{d-1} < 1$.  We model this in our GP using a projection operator $\Phi$ which imposes the constraint by sorting the vector $\vbeta$.  Applying $\Phi$ within the spatial kernel, we obtain
%on the values of the dimensions of $\vbeta$ by simply sorting the vector.  We incorporate this sorting projection into the spatial kernel
\begin{align}
    k_\beta\bigl(\bbeta, \bbeta' \bigr):=k_{S} \bigl(\Phi(\bbeta),\Phi(\bbeta') \bigr) \, .
\end{align}  
This projection does not change the value of our acquisition function, and maintains the positive definite for any covariance function for the spatial $k_S$, e.g., Matern, Polynomial.
 %yielding a permutation-invariant GP.   %to maximize the acquisition function
 We then optimize the acquisition function via a projected-gradient approach.  If a $\bbeta_t$ iterate leaves the feasible set after taking a gradient step, we project it back into the feasible set using $\Phi$ and continue. 
   We note that existing work in the GP literature has considered such projection operations in various contexts \cite{snoek2014input,van2018learning}. % maintains its positive definite form and 
 
 %, e.g. it remains an exponentiated-quadratic kernel, irrespective of this sort operation.
 %Our covariance function $k_\beta$ remains the same form of an exponentiated-quadratic irrespective the sorted input, thus it is positive semi definite for GP modeling. 
 
 %We note that existing work has exposed the use of such projection for GP in different contexts, such as warping input space for non-stationary functions \cite{snoek2014input} or learning the (unknown) invariant function from the data \cite{van2018learning}. %\vu{i've added the last 2 sentences per MAO's comment.}
%  As the GP is permutation invariant we are guaranteed that such a projection step never decreases the value of our acquisition function and is in general further from the feasible set boundary than projections under the $p$-norms typically employed in projected gradient methods. 
% \rb{GP \textit{covariance function} is permutation invariant?} \rb{is it OK to stop at `never decreases acquisition function'?}

% Recall that the vector $\vbeta=\left[\beta_{1},...,\beta_{d}\right]^T$ holds the locations of the left Riemann integral approximation in Eq. \ref{eq:left_Riemann_sum}. In order for the left Riemann approximation to the TVO to be sensible it there must be an  ordering constraint imposed on $\bbeta$ such that $0 < \beta_1 < \beta_2 < ... < \beta_d < 1$. We model this in our GP using a projection operator $\Phi$ that imposes this constraint on the values of the dimensions of $\vbeta$ by simply sorting the vector.  We incorporate this sorting projection into the spatial kernel
% \begin{align}
%     k_\beta:=k_{S} \left(\Phi(\bbeta),\Phi(\bbeta') \right)
% \end{align}  
%  yielding a permutation invariant GP.  There are multiple ways one could consider optimizing the acquisition function with such constraints.  We chose a project-gradients approach, because, when optimizing our acquisition function starting from a $\bbeta_t$ that is in the feasible set (all entries appropriately sorted) gradients of the acquisition function can easily be computed as $\Phi' = identity$ in the feasible set.  If a $\bbeta_t$ iterate leaves the feasible set after taking a gradient step while maximizing the acquisition function we project it back into the feasible set using $\Psi$ and proceed from there.  As the GP is permutation invariant we are guaranteed that such a projection step never decreases the value of our acquisition function and, is, in general, further from the feasible set boundary than projection to the feasible set under the the $p$-norms typically employed in projected gradient methods.



% The transformation function makes $k_\beta$ \textit{permutation invariant}, as any permutation of $\beta$ will result in the same covariance function after being fed through $\Phi(\bbeta)$. Equation~\ref{eq:acquisition_function} can then be optimized using a derivative-free optimizer such as coordinate descent. 


% Recall that the vector $\vbeta=\left[\beta_{1},...,\beta_{d}\right]^T$ holds the locations of the left Riemann integral approximation in Eq. \ref{eq:left_Riemann_sum}. Therefore we have an ordering constraint on $\beta$ such that $0 < \beta_1 < \beta_2 < ... < \beta_d < 1$.  



% To avoid forming $O(d^2)$ inequality constraints, we can sacrifice differentiability of the acquisition function and consider a non-differentiable transformation function $\Phi$ that sorts a d-dim vector into an increasing 1d line. We then incorporate this transformation function into the spatial kernel as
% \begin{align}
%     k_\beta:=k_{S} \left(\Phi(\bbeta),\Phi(\bbeta') \right),
% \end{align}
% where we can use any p.s.d. kernel $k_{S}$. The transformation function makes $k_\beta$ \textit{permutation invariant}, as any permutation of $\beta$ will result in the same covariance function after being fed through $\Phi(\bbeta)$. Equation~\ref{eq:acquisition_function} can then be optimized using a derivative-free optimizer such as coordinate descent. 



% In the theoretical analysis, we show that the convergence guarantee holds for popular choices of $k_{S}$, such as squared exponential or Mattern and empirically demonstrate the advantage of $k_\beta$ over $k_{S}$ in Sec. \ref{sec:Ablation_study}. 

% The benefit of permutation invariance can be seen by considering that a single evaluation of $f_{t}(\beta_{t})$ generalized to \textit{all} other permutation $f_{t}\left(\rho_i(\beta_t)\right)\forall\rho_i$, where $\rho_i :\mathbb{R}^d \to \mathbb{R}^d$ is the permutation operator. In other words, permutation invariance via $\Phi$ naturally provides the valuable information of $d!$ observations per reward.



% \subsection{Permutation Invariant S \vu{It is specific for GP. The header should be: Per Inv GP}}\label{sec:perm_invar}


%\vu{flow: placement in 1d make $\beta$ permutation invariant for evaluating $f(\beta)$-> we enable GP to handle Per Inv via $k_S$ and using projection $\Phi$}


% Recall that the vector $\vbeta=\left[\beta_{1},...,\beta_{d}\right]^T$ holds the locations of the left Riemann integral approximation in Eq. (\ref{eq:left_Riemann_sum}). Therefore, we have an ordering constraint on $\beta$ such that $0 = \beta_1 < \beta_2 < ... < \beta_{d} = 1$.

% that each value of $\beta_i$ is naturally placed in a one-dimensional line (see Fig. \ref{fig:tvo}). This placement makes our reward function $f_t$ special that it becomes \textit{permutation invariant} w.r.t. the input $\vbeta_t$. Particularly, the reward function will return the same output for all permutations $f_t(\vbeta_t)=f_{t}\bigl(\rho(\vbeta_t)\bigr)\forall\rho$, where $\rho :\mathbb{R}^d \to \mathbb{R}^d$ is the permutation operator.
%\vu{the ordering constraint does not exist in this context anymore!}


%

%  \sout{While gradient-based approaches would require a set of linear constraints on $\beta_k$, we can exploit the fact that GP bandit optimization is a derivative-free method, and instead use the (non-differentiable) sort operator.} \vm{need new argument here}

% In particular, we consider a transformation function $\Phi$ that projects\footnote{it is equivalent to sorting a vector for efficient implementation.} a $d$-dim vector into an increasing one-dimensional line. We then incorporate this transformation function into the spatial kernel $k_S(\vbeta,\vbeta')$ as
% \begin{align}
%     k_\beta:=k_{S} \left(\Phi(\vbeta),\Phi(\vbeta') \right)
% \end{align}
% where we can use any p.s.d. kernel $k_{S}$. In the theoretical analysis, we show that the convergence guarantee holds for popular choices of $k_{S}$, such as squared exponential or Mattern and empirically demonstrate the advantage of $k_{\beta}$ over $k_{S}$ in Sec. \ref{sec:Ablation_study}.


% This permutation invariant is useful and could be exploited for better modeling with GP.\footnote{The standard GP \cite{Rasmussen_2006gaussian} can not handle this permutation invariant and will be sample-inefficiency.} The na\"ive approach for handling this permutation invariant is to add all permuted observations into the
% dataset. However, it restricts the scalability of GP (cubic) because the number of each permuted observation will go factorially with the dimension $d$.


% Therefore, we propose a simple, but effective, approach for modeling this permutation invariant in a GP using a transformation function $\Phi$ that projects a $d$-dim vector into an one-dimensional line. We then incorporate this transformation function into the spatial covariance function $k_S(\vbeta,\vbeta')$ as
% \begin{align}
%     k_\beta:=k_{S} \left(\Phi(\vbeta),\Phi(\vbeta') \right)
% \end{align}
% where we can use any p.s.d. covariance function $k_{S}$. This property makes $k_\beta$ \textit{permutation invariant}, as any permutation of $\beta$ will result in the same covariance function after being fed through $\Phi(\vbeta)$. The benefit of permutation invariance can be seen by considering that a single evaluation of $f_{t}(\vbeta_{t})$ generalizes to \textit{all} other permutation $f_{t}\left(\rho_i(\vbeta_t)\right)\forall\rho_i$, where $\rho_i :\mathbb{R}^d \to \mathbb{R}^d$ is the permutation operator. In other words, permutation invariance via $\Phi$ naturally provides the valuable information of $d!$ observations per reward. We empirically demonstrate the advantage of using permutation invariant GP in \S \ref{sec:Ablation_study} and in the appendix we show that the non-permutation version will result in poorer performance in training TVO.

%  In the theoretical analysis, we show that the convergence guarantee holds for popular choices of $k_{S}$, such as squared exponential or Mattern.

% against the standard GP \cite{Rasmussen_2006gaussian}.

%This property makes $k_\beta$ \textit{permutation invariant}, as any permutation of $\beta$ will result in the same covariance function after being fed through $\Phi(\vbeta)$. The benefit of permutation invariance can be seen by considering that a single evaluation of $f_{t}(\beta_{t})$ generalizes to \textit{all} other permutation $f_{t}\left(\rho_i(\beta_t)\right)\forall\rho_i$, where $\rho_i :\mathbb{R}^d \to \mathbb{R}^d$ is the permutation operator. In other words, permutation invariance via $\Phi$ naturally provides the valuable information of $d!$ observations per reward.\vm{Frank doesn't like this argument, replacements}

\subsection{Convergence Analysis} \label{sec:convergence}
In Eq.
(\ref{eq:equivalent_minregret_maxTVO}), we showed that maximizing the \gls{TVO} objective function $\mathcal{L_T}$ as a function of $\vbeta_t$ is equivalent to minimizing the cumulative regret $R_{T/w}$ by sequential optimization within the bandit framework. Here, the subscript $T/w$ refers to the number of bandit updates given the maximum epochs $T$ and the update frequency $w$ where $w \ll T$. 

We now derive an upper bound on the cumulative regret, and show that it asymptotically
goes to zero as $T$ increases, i.e., $\lim_{T\rightarrow\infty}\frac{R_{T/w}}{T}=0$.
%This demonstrates that the gap between the optimal log eve
Thus, our bandit will converge to choosing $\vbeta_{T}$ which yields the optimal value of the \gls{TVO} objective $\mathcal{L^*_T}$ for model parameters at step $T$. 


%\rb{attempt to more fully position our contribution} 
We present the main theoretical result in Theorem \ref{thm:theorem_sublinear_regret}.  
Our \gls{TVO} framework mirrors the standard time-varying GP bandit optimization, and thus inherits convergence guarantees from \citet{bogunovic2016time}.  However, as discussed in Appendix \S\ref{app:theory}, we provide a tighter bound on the mutual information gain $\gamma_{T/w}$ which may be of wider interest. %\textsc{tvgp}.

 %Our \gls{TVO} framework requires no problem-specific modification from the standard time-varying GP bandit optimization to the setting, and thusthe proof closely follows that of

%\citet{bogunovic2016time}
%he proof, given in Appendix \S\ref{app:theory}, closely follows that as  \citet{bogunovic2016time} existing 


%We present the main theoretical result in Theorem \ref{thm:theorem_sublinear_regret} \textcolor{red}{ which follows \cite{bogunovic2016time} using our tighter bound on $\tilde{\gamma}$ presented in the Appendix \S\ref{app:theory}.}

%and refer to  Appendix \S \ref{app:theoretical_analysis} for the proofs. %\vu{Frank: i have corrected $P(..\ge L_t)$, do you still want to explicitly define $L_t$}

\begin{theorem} \label{thm:theorem_sublinear_regret}
Let the domain $\mathcal{D}\subset[0,1]^{d}$ be compact and convex.  Let $L_t \ge0$ be the Lipschitz constant for the reward function at time $t$.    Assume that the covariance function $k$ is almost surely continuously differentiable, with $f\sim GP(0,k)$.  Further, for $t\le T$ and $j\le d$, we assume
 %\text{Pr} \left(\sup\left|\frac{\partial f_{t}(\vbeta_{t})}{\partial\vbeta_{t}^{(j)}}\right|\le L_{t}\right)\le ae^{-\left(L_{t}/b\right)^{2}} \quad \text {for some $a$ and $b$.}
\begin{align*}
    \text{Pr} \left(\sup\left| \partial f_{t}(\vbeta_{t}) / \partial\vbeta_{t}^{(j)}\right|\ge L_{t}\right)\le ae^{-\left(L_{t}/b\right)^{2}} \quad 
\end{align*}
for appropriate choice of $a$ and $b$ corresponding to $L_t$.
%$\forall L_t \ge0$ which is a Lipschitz constant for our reward function at time $t$.

For $\delta\in(0,1)$, we write  $\kappa_{T/w}=2\log\frac{\pi^{2}T^{2}}{2\delta w^2}+2d\log db{\frac{T^{2}}{w^2}} \sqrt{\log\frac{da\pi^{2}T^{2}}{2\delta w^2}}$
and $C_{1}=8/\log(1+\sigma_{f}^{2})$.  Then, after $T/w$ time steps, our algorithm satisfies %the following
\begin{align*}
R_{T/w}=\sum_{t=1}^{T/w}f_{t}(\vbeta_{t}^{*})-f_{t}(\vbeta_{t}) & \le\sqrt{\gamma_{T/w} \cdot C_{1} \cdot \kappa_{T/w} \cdot T/w}+2
\end{align*}
% \begin{align*}
% R_{T/w}=\sum_{t=1}^{T/w}f_{t}(\vbeta_{t}^{*})-f_{t}(\vbeta_{t}) & \le\sqrt{\gamma_{\frac{T}{w}} \cdot C_{1} \cdot \kappa_{T} \cdot T/w}+2
% \end{align*}
%\le\sqrt{C_{1}T\kappa_{T}\gamma_{T}}+2
with probability at least $1-\delta$, where $\gamma_{T/w}$ is the maximum information gain for the time-varying covariance function (see below). %The bound holds for any $\tilde{N}\in\left\{ 1,...,T/w\right\} $.
\end{theorem}
% \begin{align*}
%     \text{Pr} \left(\sup\left| \partial f_{t}(\vbeta_{t}) / \partial\vbeta_{t}^{(j)}\right|\ge L_{t}\right)\le ae^{-\left(L_{t}/b\right)^{2}} \quad \text {for some $a$ and $b$.}
% \end{align*}
% $\forall L_t \ge0$ which is a Lipschitz constant for our reward function at time $t$. Let $\delta\in(0,1)$,   $\kappa_{T}=2\log\frac{\pi^{2}T^{2}}{2\delta}+2d\log dbT^{2}\sqrt{\log\frac{da\pi^{2}T^{2}}{2\delta}}$, and $C_{1}=8/\log(1+\sigma_{f}^{2})$.  After $T$ time steps, our algorithm
% satisfies
% \begin{align*}
% R_{T/w}=\sum_{t=1}^{T/w}f_{t}(\vbeta_{t}^{*})-f_{t}(\vbeta_{t}) & \le\sqrt{\gamma_{T/w}C_{1}\kappa_{T}T/w}+2
% \end{align*}


%kernel) for modeling $\vbeta$
% , so that $k_S \propto \exp\bigl(-\frac{1}{2 \phi^2}(\cdot- \cdot)^2\bigr)$ for $\phi$ a hyperparameter,
%\rb{expression in sentence 1 appears in Thm/Lemma in App?} \rb{base covariance?  = kernel?} \vu{yes}
%\vu{Mike wrote it: Using an exponentiated-quadratic base covariance for $\vbeta$  so that $k_S \propto \exp\bigl(-\frac{1}{2 \phi^2}(\cdot- \cdot)^2\bigr)$ for $\phi$ a hyperparameter. But, it is super confused as we (unneccessarily) introduce $\phi$ which is overwritten by our $q_{\phi}$. So I have remove it.} 


% \begin{align*}
% R_{T/w}=\sum_{t=1}^{T/w}f_{t}(\vbeta_{t}^{*})-f_{t}(\vbeta_{t}) & \le\sqrt{\left(1+ T / \left[w \tilde{N} \right]\right) \left(\gamma^{\vbeta}_{\tilde{N}}+\sigma_{f}^{-2}\tilde{N}^{5/2}\omega\right)C_{1}\kappa_{T}T/w}+2
% \end{align*}
In the above theorem, the quantity $\gamma_{T/w}$ measures the maximum information gain obtained about the reward function after pulling $T/w$ arms \cite{Srinivas_2010Gaussian, bogunovic2016time}. %for a specific kernel over $x = [\vbeta, t]$. %using a specific choice of covariance function for $k_{\beta}$.
%In$\gamma_{T/w}$ provides the meaningful quantity over the maximum information we can gain after pulling $T/w$ arms using a specific choice of covariance function for $k_{\beta}$.
%$\gamma_{T/w}=\left(1+ T / \left[w \tilde{N} \right]\right) \left(\gamma^{\vbeta}_{\tilde{N}}+\sigma_{f}^{-2}\tilde{N}^{5/2}\omega\right)$ ....
In the Appendix \S\ref{app:theory}, we show that $\gamma_{T/w} \le \left(1+ T / \left[w \tilde{N} \right]\right) \left(\gamma^{\vbeta}_{\tilde{N}}+\sigma_{f}^{-2}\tilde{N}^{5/2}\omega\right)$,
where $\tilde{N}\in\left\{ 1,...,T/w\right\}$ denotes a time-varying block length, and $\gamma^{\vbeta}_{\tilde{N}}$ is defined with respect to the covariance kernel for $\vbeta$. 
For our particular choice of exponentiated-quadratic kernel, the maximum information gain scales as $\gamma^{\vbeta}_{\tilde{N}} \le  \mathcal{O}( \log \tilde{N}^{d+1})$ \cite{Srinivas_2010Gaussian}. 
%\rb{clarify $\gamma_{T/w}$ vs. $\gamma^{\vbeta}_{\tilde{N}}$ in referencing MI gain?} 
Compared with \cite{bogunovic2016time}, our proof tightens the upper bound on $\gamma_{T/w}$ from $\mathcal{O}(\tilde{N}^{3})$ to $\mathcal{O}(\tilde{N}^{5/2})$.

Combining these terms, we can then write the bound as $R_{T/w} \lesssim \mathcal{O}(\sqrt{\left( \left[ \log \tilde{N}^{d+1} + \sigma_{f}^{-2}\tilde{N}^{5/2}\omega\right] T/w \right)}$, which is sublinear in $T$ when the function $f$ becomes time-invariant, i.e.,  $\omega \rightarrow 0$. In contrast, the sublinear guarantee does not hold when the time-varying function is non-correlated, i.e., $\omega=1$, in which case the time covariance matrix becomes identity matrix. The bound is tighter for lower schedule dimension $d$.%. and forgetting parameter $\omega$, with $\omega=0$ reducing to a time-invariant function.

% Combining these terms, we can then write the bound as $R_{T/w} \lesssim \mathcal{O}(\sqrt \left(  \left[\log \tilde{N}^{d+1} + \sigma_{f}^{-2}\tilde{N}^{5/2}\omega\right] T/w} \right)$, which is sublinear in $T$. The bound is tighter for both lower schedule dimension $d$ and forgetting parameter $\omega$, with $\omega=0$ reducing to a time-invariant function.

%and \vu{for a time-varying block} $\tilde{N}\in\left\{ 1,...,T/w\right\} $
 %=\left(1+ T / \left[w \tilde{N} \right]\right) \left(\gamma^{\vbeta}_{\tilde{N}}+\sigma_{f}^{-2}\tilde{N}^{5/2}\omega\right)$
% *** PREVIOUS ***
% Using an exponentiated-quadratic base covariance for $\vbeta$, we have the maximum information gain bound as $\gamma^{\vbeta}_{\tilde{N}} \le  \mathcal{O}( \log \tilde{N}^{d+1})$ \cite{Srinivas_2010Gaussian}. The maximum information gain for the product of time covariance function and exponentiated-quadratic, derived in Lem. \ref{lem:bound_MIG_timevarying} in the Appendix, is included in Theorem \ref{thm:theorem_sublinear_regret}. Overall, we can 
% write the bound as $R_{T/w} \lesssim \mathcal{O}(\sqrt \left(  \left[\log \tilde{N}^{d+1} + \sigma_{f}^{-2}\tilde{N}^{5/2}\omega\right] Tw^{-1} \right)$ which is sublinear in $T/w$. The bound is loose for high dimension $d$ and for increased forgetting parameter $\omega$.


\begin{figure*}
\includegraphics[width=0.33\columnwidth]{fig/reward_func_S50_epoch1000.pdf}
\includegraphics[width=0.33\columnwidth]{fig/reward_func_S50_epoch2000.pdf}
\includegraphics[width=0.33\columnwidth]{fig/reward_func_S50_epoch9000.pdf}
\caption{Time-varying reward function $f_t(\bbeta_t)$ after 2k, 3k, and 10k training epochs, with bandit choices of a single intermediate $\beta_1$ (i.e. $\vbeta = [0, \beta_1]$) colored by timestep.  Scattered $\beta_1$ in neighboring epochs indicate `exploration', while similarly colored values of $\beta_1$ in regions where the GP mean, or predicted reward, is high indicate `exploitation'. 
%with $\vbeta = [0, \beta_1]$.  Color encodes timestep
%across training epochs for a single $\vbeta = [0, \beta_1]$. We consider the case of optimizing a single $\vbeta = [0, \beta_1]$ for visualization purposes, with colored dots reflecting $\beta_1$ choices within given epoch windows.  Similar values of $\beta_1$ with the same color indicate that the bandit is exploiting performance in a given $[\vbeta, t]$ region. As the objective converges near the end of training, our GP adapts to have low variance and the choice of $\beta_1$ is less significant.
% Example of the time-varying reward functions of $f_t(\bbeta_t)$ at three different period in time. We consider the case of optimizing a single $\vbeta = [0, \beta_1]$ for visualization purposes, with colored dots reflecting $\beta_1$ choices within given epoch windows.  Similar values of $\beta_1$ with the same color indicate that the bandit is exploiting performance in a given $[\vbeta, t]$ region. As the objective converges near the end of training, our GP adapts to have low variance and the choice of $\beta_1$ is less significant.
} \label{fig:exmaple_time_reward}%heteroskedastic
%\vspace{-1pt}
\end{figure*}



==> framework_backup.tex <==
\section{From Evidence Maximization to Regret Minimization}\label{sec:bandits}
\begin{figure*}
\includegraphics[width=0.33\columnwidth]{fig/function_S10.pdf}
\includegraphics[width=0.33\columnwidth]{fig/function_S50.pdf}
\includegraphics[width=0.33\columnwidth]{fig/function_S100.pdf}
\caption{Example of the time-varying reward functions $f_t(\bbeta_t)$ using different $S=10,50,100$ estimated within the same epoch range from $2000-3000$.  The high level of noise makes the gradient-based approach inappropriate.   \label{fig:exmaple_function_S}}

\end{figure*}

\vm{Vu give this paragraph another scan w/ the new changes to see if I've addressed your comments. Just added a few extra words here and there}
We view the vector $\bbeta \in [0,1]^d$ as an arm \cite{Auer2002nonstochastic} to be pulled in a continuous space, given a fixed resource of $T$ training epochs. After each round, we receive with an estimate of the log evidence, given by Eq. (\ref{eq:left_Riemann_sum}), from which we will construct a reward function. An important feature of our problem is that the \gls{TVO} updates of $\theta_t, \phi_t$ cause the integrand in \cref{fig:tvo} to change between rounds as the \gls{TVO} converges. Thus, our multi-armed bandit problem is said to be \textit{time-varying}, in that the optimal arm and reward function depend on round $t$.


 
% \vm{Vu I added ``as the TVO converges'' to indicate the $\theta_t, \phi_t$ updates are due to tvo convergence. I think the rest of your comment would fit better in the experimental section when we can empirically observe that $\beta=0$ gives high reward at earlier stages}

% \vu{the second cause would be from the convergence of TVO, at different stages of TVO training, the behavior of our reward function would be different, e.g., $\beta=0$ gives high reward at earler stage, but $\beta=1$ does at later stage}

More formally, we define the time-varying reward function $f_{t}:[0,1]^{d}\rightarrow\mathcal{R}$ which takes an input $\bbeta_{t}$ and produces reward $f_{t}(\bbeta_{t})$. At each round we get access to a noisy reward, or utility ${u_t=f_{t}(\bbeta_{t})+\epsilon_t}$ where we assume Gaussian noise $\epsilon_{t}\sim\mathcal{N}(0,\sigma_{f}^{2})$. We aim to maximize the cumulative reward $\sum_{t=1}^{T/w}f_{t}(\bbeta_{t})$ across $T/w$ rounds, where $w$ is an integer multiple of $T$ and will later control the ratio of bandit rounds to training epochs.

Maximizing the cumulative reward is equivalent to minimizing the \textit{cumulative regret}
\begin{align}
    R_{T/w} = \sum_{t=1}^{T/w} f_{t}(\bbeta_t^*) - f_{t}(\bbeta_t) \label{eq:cumulative_regret}
\end{align}
where $r_t = f_{t}(\bbeta_t^*) - f_{t}(\bbeta_t)$ is the \textit{instantaneous regret} defined by the difference between the received reward $f_{t}(\bbeta_t)$ and maximum reward attainable $ f_{t}(\bbeta_t^*)$ at round $t$. The regret, which is non-negative and monotonic, is more convenient to work with than the cumulative reward and will allow us to derive upper bounds on the regret in Section \ref{sec:convergence}.

In order to translate the problem of maximizing the log evidence into the bandits framework, we must construct the time-varying reward function $f_t(\bbeta_t)$ in such a way that minimizing the cumulative regret it is equivalent to maximizing the final \gls{TVO} epoch, i.e such that $\min R_{T/w} = \max \mathcal{L}_T$.

Such a reward function can be defined by partitioning the $T$ training epochs into windows of equal length $w$, and defining the reward for each window $t \in \{1, 2, ..., T/w\}$
\begin{align}
    f_{t}(\bbeta_{t}):=\mathcal{L}_{wt} - \mathcal{L}_{w(t-1)}\label{eq:reward_function}
\end{align}
by the window-length difference in \gls{TVO} log evidence estimates. Then, the cumulative reward is given by a telescoping sum over windows 
\begin{align}
\sum_{t=1}^{T/w}f_{t}(\bbeta_{t}) &= (\mathcal{L}_{w} - \mathcal{L}_{0}) + (\mathcal{L}_{2w} - \mathcal{L}_{w}) + ... + (\mathcal{L}_{(T/w)w} - \mathcal{L}_{(T/w~-1)w})\\
                                  &= \mathcal{L}_T - \mathcal{L}_0, \label{eq:cumulative_reward_function}
\end{align}
where $\mathcal{L}_0$ is the initial (i.e. untrained) loss. Recalling the definition of cumulative regret in \cref{eq:cumulative_regret}
\begin{align} \label{eq:equivalent_minregret_maxTVO}
    \min R_{T/w} &= \min \sum_{t=1}^{T/w} f_{t}(\bbeta_t^*) - f_{t}(\bbeta_t) \\ 
    &= \min\left(\sum_{t=1}^{T/w}f_{t}(\bbeta_t^*)\right) - \left(\sum_{t=1}^{T/w}f_{t}(\bbeta_t)\right)\\
                 &= \min\left(\left(\mathcal{L}^*_T - \mathcal{L}_0\right) - \left(\mathcal{L}_T - \mathcal{L}_0\right)\right)  \\
                 &= \min~(\textit{const} - \mathcal{L}_T) \\
                 &= \max\mathcal{L}_T.
\end{align}
Therefore minimizing the cumulative regret for the reward function defined by \cref{eq:reward_function} is equivalent to maximizing the log evidence in the TVO. Next, we describe how to design an optimal decision mechanism to minimize the cumulative regret $R_{T/w}$ using Gaussian processes.
%\rb{Is it possible to rewrite something in terms of TVO here? Just for extra clarity before we dive fully into $f(\beta_t)$} 
% \begin{lem}
% \label{lem:equivalent_maxlogpx_min_regret} Let $\bbeta=[\beta_{1},...\beta_{d}]\in[0,1]^{d}$
% and define the oracle $\mathcal{L}_T^{*}$
% which is the best we can get $\mathcal{L}_T^{*}:=\sum_{t=1}^{T}f_{t}^{*}$
% where $f_{t}^{*}=\max_{\forall\bbeta}f_{t}(\bbeta)$ is the global
% optimum of the reward function at time step $t$. We show that maximizing
% the log evidence of TVO $\mathcal{L}_T$ is equivalent to minimizing the cumulative
% regret $R_T=\sum^T_{t=1} f^*_t - f_t(\bbeta_t)$ in the time-varying bandit problem.
% \begin{align*}
% \max\mathcal{L}_T-\textrm{const} & =\min\left(\mathcal{L}_T^{*}-\mathcal{L}_T+\mathcal{L}_0\right)=\min\sum_{t=1}^{T}\underbrace{f_{t}^{*}-u_{t}}_{\textrm{regret}}=\min R_{T}.
% \end{align*}
% \end{lem}

% \begin{proof}
% $\mathcal{L}_T^*-\mathcal{L}_0$ is a constant, we achieve the above derivations by using Eq. (\ref{eq:equivalent_logpT_cumregret}).
% \end{proof}
% We have derived the equivalence between the main goal of maximizing the
% log evidence in TVO to minimizing the cumulative regret. Under this
% novel view, we can develop a GP bandit optimization \cite{Srinivas_2010Gaussian,bogunovic2016time} to sequentially optimize $\bbeta$  and show that the result will lead to the optimal solution, satisfying condition \textcolor{blue}{\textcircled{\small{2}}}.


% \subsection{Time-varying GP bandit for sequentially selecting $\beta_{1...d}$}


\section{Time-varying GP Bandit Optimization}\label{sec:gp}

Using GP for bandit optimization, we first define the time-varying Gaussian process as the surrogate model over the time-varying reward function. We then extend the time-varying GP to handle input permutation invariant as the property of the 1D integration in TVO. Next, we describe the acquisition function used to select the next $\bbeta_t$. Finally, we derive the convergence analysis which provides the theoretical guarantee that the chosen integration schedule $\bbeta_t$ will lead to the optimal result asymptotically.

%We formulate it as a time-varying Gaussian process bandit optimization in \S \ref{sec:TVGP} since our continuous reward function is a black-box function which is expensive, non convex and  time-varying. 


%We below present a surrogate model using an extension of a Gaussian process \cite{Rasmussen_2006gaussian} for handling permutation invariant input and a decision function to select $\bbeta_t$.  Finally, we derive the convergence analysis and show that the chosen point $f_{t}(\bbeta_{t})$ will lead to the optimal result $f_{t}(\bbeta_{t}^{*})$ asymptotically.

\subsection{Time-varying Gaussian process} \label{sec:TVGP}



We develop the permutation invariant time-varying Gaussian process model. We first describe the time-varying GP. We then explain why we need permutation invariant GP and present the new model. 

A popular design in handling time-varying function is jointly modeling the spatial and temporal parameter using a product form of the kernel \cite{Krause_2011Contextual,Swersky_2013Multi,klein2017fast,nyikosa2018adaptive}. Under this joint modeling framework, the time-varying reward function will be assumed to follow a GP as $f_t \sim GP(0, k(\bbeta,\bbeta')\times k(t,t'))$ where we have considered zero mean for simplicity. Using a conditioning property \cite{Bishop_2006pattern}, we estimate the predictive distribution \cite{Rasmussen_2006gaussian} at any input $\bbeta_{*}$ at time step $t$  as $p_t(\bbeta_{*}) \sim \mathcal{N} \left( \mu_t(\bbeta_{*}), \sigma_t(\bbeta_{*}) \right)$ where  \vspace{-15pt}

\begin{minipage}[t]{0.48\columnwidth}%
\begin{align}
\mu_t\left(\bbeta_{*}\right)= & \mathbf{\bk}_{*}\left[\mathbf{K}+\sigma_{f}^{2}\idenmat\right]^{-1}\mathbf{u}\label{eq:mu_f_per_inv}
\end{align}
%
\end{minipage}%
\begin{minipage}[t]{0.48\columnwidth}%
\begin{align}
\sigma_t^{2}\left(\bbeta_{*}\right)= & k_{**}-\mathbf{\bk}_{*}\left[\mathbf{K}+\sigma_{f}^{2}\idenmat\right]^{-1}\mathbf{\bk}_{*}^{T}\label{eq:sigma_f_per_inv}
\end{align}
%
\end{minipage}

where $\bu=[u_{i}]_{\forall i\le t}$, $\ensuremath\bk_{*}=[k\left(\bv_{*},\bv_{i}\right)]_{\forall i}$,
$\ensuremath{\mathbf{K}=\left[k\left(\bv_{i},\bv_{j}\right)\right]_{\forall i,j}}$,
$\ensuremath{k_{**}=k\left(\bv_{*},\bv_{*}\right)}$, $\bv_*=\left[ \bbeta_{*}, t \right]$,
$\sigma_{f}^{2}$ is the noise variance for $f$ and $k(\bv_{i},\bv_{j})=k_{\beta}\left(\bbeta_{i},\bbeta_{j}\right)\times k_{time}\left(t,t'\right)$, $k_\beta$ and $k_{time}$ are the covariance functions for $\bbeta$ and $t$ respectively. For convenience in the theoretical analysis, we follow \cite{bogunovic2016time} to use a specific choice of $k_{time}(t,t')=(1-\omega)^{\frac{|t-t'|}{2}}$ where $\omega$ is the forgetting-remembering parameter trade-off which is learnt from the data. We next discuss on how to model the $k_\beta$ for permutation invariant property.
%$\omega$ is a hyperparameter for the time-varying kernel.

%$k(\bv_{i},\bv_{j})=k_{\beta}\left(\Phi\left(\bbeta_{i}\right),\Phi\left(\bbeta_{j}\right)\right)\times(1-\omega)^{\frac{|i-j|}{2}}$

\subsection{Input Permutation Invariant for Time-varying GP}

In our TVO setting, the values in a $d-$dimensional vector $\bbeta=\left[\beta_{1},...,\beta_{d}\right]\in\left[0,1\right]^{d}$
will be used to estimate the 1-dimensional integral in Eq. (\ref{eq:left_Riemann_sum}). This property makes our reward function is \textit{permutation invariant} (see Lemma \ref{lem:permutation_invariant}) that raises challenges for any gradient-based approach \vu{any supporting evidence, explanation or citation?}. On the other hand, as a derivative-free method, our GP bandit optimization is resilient to such ordering constraints.

As opposed to the gradient-based approach, this permutation invariant property is useful and could be exploited for better modeling for the GP. The benefit of such permutation invariant can be seen as follows: by observing a single evaluation of $f_{t}(\beta_{t})$,
we can generalize to all other permutation of $\bbeta_{t}$, $f_{t}([\beta_{1},...,\beta_d])=f_{t}\left([\beta_{\rho(1)},...,\beta_{\rho(d)}]\right)\forall\rho$
where $\rho$ is the permutation operation. In other words, the permutation invariant naturally shows the valuable information of $d!$ number of observations where $d$ is the dimension of $\bbeta$. %, i.e., $f_{t}(\bbeta_{t}=[\beta_{1},...,\beta_{K}])=f_{t}\left([\beta_{\rho(1)},...,\beta_{\rho(d)}]\right)\forall\rho$ where $\rho$ is the permutation operation.

%By projecting into $1-$dimensional integral, we have an interesting property that $0\le\beta_{1}\le\beta_{2}\le...\le\beta_{d}\le1$. 



\begin{lem} \label{lem:permutation_invariant}
The time-varying reward function $f_{t}(\bbeta_t)$ in TVO is permutation invariant
w.r.t. the input.
\end{lem}

\begin{proof}
We use a $d-$dimensional vector of $\bbeta=[\beta_{1},...,\beta_{d}]$ to estimate the 1D integral in Eq. (\ref{eq:left_Riemann_sum}). This
is equivalent to project a $d-$dimensional vector into a line
with an increasing order, such that $0\le\beta_{1}\le\beta_{2}\le...\le\beta_{d}\le1$.
We therefore have that $f_{t}([\beta_{1},...,\beta_d])=f_{t}\left([\beta_{\rho(1)},...,\beta_{\rho(d)}]\right)\forall\rho$
where $\rho$ is the permutation operation.
\end{proof}

For handling this permutation invariant, the na\"ive approach is to add all permuted observations into the
dataset. However, the number of permuted observations will go factorially with the dimension and the GP complexity grows cubically with the observations. Therefore, this approach is not scalable with respect to $d$ and large number of epoch $T$.

% to the standard time-varying GP for modeling this permutation invariant property. 

%a good GP should be able to generalize to all of permutations of $\bbeta$. Modeling using the vanilla GP may fail to capture this special property.

%, e.g., when $d=5$ dimensions, each $\bbeta$ will generate $5!=120$ permuted betas

Therefore, we propose a simple, but effective, approach for modeling this permutation invariant (time-varying) GP without the need of storing all of the permuted variables while achieving the desired property. Particularly, we consider a transformation function $\Phi$ which projects $d-$dimensional vector $\bbeta$ into a 1-dimensional line. This projection can be done by sorting K-dim
vector into an increasing 1d line. We then incorporate this transformation function into the covariance function as $k_\beta:=k_{\beta} \left(\Phi(\bbeta),\Phi(\bbeta') \right)$ where we can use $k_\beta$ as any p.s.d. covariance function. In the theoretical analysis, we show that the convergence guarantee holds for popular choices of $k_\beta$ kernel, such as squared exponential or Mattern. We demonstrate the advantage of our proposed permutation invariant GP modeling in Sec. \ref{sec:Ablation_study} against the standard GP \cite{Rasmussen_2006gaussian}.
% Under this projection, we ensure that our kernel is permutation invariant while we don't need to physically add permuted data points into the dataset.

%The advantage of this approach is that we don't need to store all of the permuted variables in the dataset while we obtain the desired property.


We optimize the GP hyperparameters (such as length-scale and noise
variance) of $K$ by maximizing the marginal likelihood \cite{Rasmussen_2006gaussian}. We describe
the gradient of $\omega$ in the appendix.

Our permutation invariant GP is related to \cite{van2018learning} which aims to learn the unknown invariant function from the data. In our 1D integration setting, it is much simpler as the invariant function $\Phi$ of 1D ordering is known in advance.

\subsection{Acquisition function for selecting the next schedule $\beta_t$} \label{sec:acquisition_function}

Using the above permutation invariant time-varying GP as a surrogate model for the reward function, we next define an acquisition function
to sequentially select the next $\bbeta_t$. While there could be different
types of acquisition functions available \cite{Jones_1998Efficient,Hennig_2012Entropy,Hernandez_2014Predictive},
we follow the time-varying version of GP-UCB \cite{Srinivas_2010Gaussian,bogunovic2016time} which allows us to
derive the convergence analysis. Particularly, we select
\begin{align}
\bbeta_{t}= & \arg\max_{\bbeta}\,\alpha_{t}(\bbeta) = \arg\max_{\bbeta}\mu_{t}(\bbeta)+\sqrt{\kappa_{t}}\sigma_{t}(\bbeta) ,\forall t=1,....,T \label{eq:acquisition_function}
\end{align}

where $\mu_t(\bbeta)$ and $\sigma_t(\bbeta)$ are from Eqs. (\ref{eq:mu_f_per_inv},\ref{eq:sigma_f_per_inv}),  $\kappa_{t}$ is the exploration-exploitation trade-off parameter that we can theoretically set $\kappa_{t}$ in Theorem \ref{thm:theorem_sublinear_regret} for convergence guarantee. The acquisition function in Eq. (\ref{eq:acquisition_function}) can be optimized efficiently by any global optimization toolbox, such as multi-start BFGS \cite{fletcher2013practical} or DIRECT \cite{Jones_1993Lipschitzian}, because $\alpha_t(\bbeta)$ is cheap to compute and gradient available \cite{Rasmussen_2006gaussian}. 

% \paragraph{Regret.}
% A natural performance metric in this context is cumulative regret,
% the loss in reward due to not knowing the maximum points of the black-box
% function beforehand. Suppose the unknown function is f, its maximum
% point $\bx_t^{*}=\arg\max_{\bx_\in D}f_t(\bx)$. For our choice $\bx_{t}$
% in iteration $t$, we incur instantaneous regret $r_{t}=f_t\left(x_t^{*}\right)-f_t\left(x_{t}\right)$.
% The cumulative regret $R_{T}$ after $T$ iterations is the sum of
% instantaneous regrets: $R_{T}=\sum_{t=1}^{T}r_{t}$. A desirable asymptotic
% property of an algorithm is to be no-regret: $\lim_{T\rightarrow\infty}\frac{R_{T}}{T}=0$.
% Note that neither $r_{t}$ nor $R_{T}$ are ever revealed to the algorithm.



\begin{algorithm}
\caption{TVO-GPTV (high level)\label{alg:TVO_GPTV_highlevel}}

\begin{algor}
\item [{{*}}] Input: the reward function $f_{t}(\bbeta_{t})$, $d$ is
dimension of $\bbeta$
\end{algor}
\begin{algor}[1]
\item [{for}] $t=1....T$
\item [{{*}}] Train the TVO objective function given $\bbeta_{t-1}$ obtained
previously
\item [{if}] time to update $\bbeta_t$ or mod(t,w)=0
\item [{{*}}] Estimate the utility $u_{t}=\mathcal{L}_{t}-\mathcal{L}_{t-w}$ and augment
$D_{t+1}=D_{t}\cup\left(\bbeta_{t-1},t,u_{t}\right)$
\item [{{*}}] Fit a time-varying, permutation invariant GP to $D_{t}$ to estimate $\mu_{t}(\bbeta),\sigma_{t}(\bbeta)$ from Eqs.
(\ref{eq:mu_f_per_inv},\ref{eq:sigma_f_per_inv}) 
\item [{{*}}] Select $\bbeta_{t}=\arg\max \mu_{t}(\bbeta)+\sqrt{\kappa_{t}}\sigma_{t}(\bbeta)$ where $\kappa_{t}$ is from Theorem \ref{thm:theorem_sublinear_regret}.
\item [{endif}]~
\item [{endfor}]~
\end{algor}
\end{algorithm}

% {\forall\bbeta\in\left[0,1\right]^{d}}

\subsection{Convergence Analysis} \label{sec:convergence}
In Eq.
(\ref{eq:equivalent_minregret_maxTVO}), we show that maximizing the TVO objective function $\mathcal{L_T}$ is equivalent to minimize the cumulative regret $R_{T}$ defined by sequentially optimize $\bbeta_{t}$ in the bandit setting. We now derive
the upper bound over the cumulative regret $R_T$ and show that it asymptotically
goes to zero as $T$ increases, i.e., $\lim_{T\rightarrow\infty}\frac{R_{T}}{T}=0$.
Due to the equivalence, this upper bound quantifies the gap between the optimal log evidence we can achieve $\mathcal{L^*_T}$ and our obtained log evidence $\mathcal{L_T}$ by the bandit. Specifically, our chosen $\bbeta_{t},\forall t$ will lead to the TVO converging to the optimal one.

We present the main theoretical result in Theorem \ref{thm:theorem_sublinear_regret} and refer to the appendix for the proofs. \vu{any idea on writing this theorem correctly, but not as ugly as it is now :)}

%We make the following smoothness assumption to derive the regret bound of the proposed algorithm.

% \textbf{Assumptions.}

% We will assume that the kernel $k$ is such that a (strict) subset
% of the following statements hold for some $\left(a,b\right)$ and
% all $L\ge0$.
% \begin{enumerate}
% \item The time kernel satisfies $1-k_{time}(t,t')\le\omega\left|t-t'\right|$
% for some $\omega\in\left[0,1\right]$ and for any $t,t'\in\mathcal{T}$.
% \item The joint kernel satisfies for $j=1,...,d,$
% \begin{align}
% \forall L & \ge0,t\le\mathcal{T},p\left(\sup\left|\frac{\partial f_{t}(\bbeta_{t})}{\partial\bbeta_{t}^{(j)}}\right|\le L_{t}\right)\le ae^{-\left(L_{t}/b\right)^{2}}.\label{eq:Lipschitz_assumption}
% \end{align}
% \end{enumerate}
% The assumption 1 is achieved by using a time-varying kernel $k_{time}(t,t')=\left(1-\omega\right)^{\frac{|t-t'|}{2}}$
% \cite{bogunovic2016time}. We below prove that the assumption 2 is
% satisfied.

% \vu{Vaden will include the discussion on the common assumption on this Lipschitz, but we dont need to make it as a lemma}

% \begin{lem}
% \label{lem:Lipschitz}We show that the TVO likelihood function controlled
% by $\bbeta$ is Lipschit continuous:

% $p(\sup\left|\frac{\partial f_{t}(\bbeta_{t})}{\partial\bbeta_{t}^{(j)}}\right|\le L)\le ae^{-\left(L/b\right)^{2}}$
% for $j=1,...,d$ \forall L & \ge0,t\le\mathcal{T},p\left(\sup\left|\frac{\partial f_{t}(\bbeta_{t})}{\partial\bbeta_{t}^{(j)}}\right|\le L_{t}\right)\le ae^{-\left(L_{t}/b\right)^{2}}.
%\label{eq:Lipschitz_assumption}

% Proof: to be done by Vaden.
% \end{lem}

% Let the time kernel satisfies $1-k_{time}(t,t')\le\omega\left|t-t'\right|$ for some $\omega\in\left[0,1\right]$ and for any $t,t' \le T$. 

%We summarize the main theoretical result and refer to the appendix for all detailed derivations.
\begin{thm} \label{thm:theorem_sublinear_regret}
Let the domain $\mathcal{D}\subset[0,1]^{d}$ be compact and convex, the kernel $f\sim GP(0,k)$ is almost
surely continuously differentiable and satisfies  $\forall L \ge0$,$t\le T,j\le d,p\left(\sup\left|\frac{\partial f_{t}(\bbeta_{t})}{\partial\bbeta_{t}^{(j)}}\right|\le L_{t}\right)\le ae^{-\left(L_{t}/b\right)^{2}}$ 
for some $a$ and $b$. Let $\delta\in(0,1)$, $\kappa_{T}=2\log\frac{\pi^{2}T^{2}}{2\delta}+2d\log dbT^{2}\sqrt{\log\frac{da\pi^{2}T^{2}}{2\delta}}$, and $C_{1}=8/\log(1+\sigma_{f}^{2})$, our algorithm
satisfies the following after $T$ time steps:
\begin{align*}
R_{T}=\sum_{t=1}^{T}f_{t}(\bbeta_{t}^{*})-f_{t}(\bbeta_{t})\le\sqrt{C_{1}T\kappa_{T}\gamma_{T}}+2 & \le\sqrt{C_{1}T\kappa_{T}\left(\frac{T}{\tilde{N}}+1\right) \left(\gamma^{\beta}_{\tilde{N}}+\frac{1}{\sigma_{f}^{2}}\tilde{N}^{5/2}\omega\right)}+2
\end{align*}
with probability at least $1-\delta$, where $\gamma^{\beta}_{\tilde{N}}$ is the maximum information gain of the kernel for modeling $\bbeta$. The bound holds for any
$\tilde{N}\in\left\{ 1,...,T\right\} $.
\end{thm}

When modeling $\bbeta$ using squared exponential kernel, we have the maximum information gain bound as $\gamma^{\beta}_{\tilde{N}} \le  \mathcal{O}( \log \tilde{N}^{d+1})$ \cite{Srinivas_2010Gaussian}. Then, we can plug this $\gamma^{\beta}_{\tilde{N}}$ into Theorem 3 to see $\lim_{T\rightarrow\infty}\frac{R_{T}}{T}=0$.


% Our theoretical analysis assumed that we know the hyperparameters of both spatial (lengthscale $\sigma_{l}^{2}$ for squared exponential kernel), temporal kernel ($\omega$) and noise variance $\sigma^2_f$. Having perfect knowledge of and other hyperparameters is typically not realistic. The GP perspective allows us to select them in a principled way by maximizing the GP marginal likelihood


==> vu_back_up_writing.tex <==

\section{Time-varying Gaussian Process Bandit Preliminaries}

\vu{this section could be later remove.}
Many applications require optimizing an unknown, noisy function that
is expensive to evaluate. This optimization can be formalized as a
continuous multi-armed bandit problem, where the payoff function is
typically sampled from a Gaussian process (GP) \cite{Srinivas_2010Gaussian,bogunovic2016time}.

Time-varying bandit optimization extends the above sequential optimization
with bandit feedback for handling the reward function which varies
with time \cite{bogunovic2016time}. Formally, we seek to sequentially
optimize an unknown reward function $f_{t}$ over a compact, convex
subset $D\subset\mathcal{R}^{d}$. At time $t$, we can interact with
$f_{t}$ only by querying at some point $\bx_{t}\in D$ after which
we observe a noisy observation $y_{t}=f_{t}(\bx_{t})+\epsilon_{t}$,
where $\epsilon\sim\mathcal{N}\left(0,\sigma_{f}^{2}\right)$.

The goal is to maximize the reward via a suitable trade-off between
exploration and exploitation. This problem is ill-posed for arbitrary
reward functions even in the time-invariant setting, and it is thus
necessary to introduce suitable smoothness assumptions. For example,
Bogunovic et al \cite{bogunovic2016time} model the reward function
as a sample from a Gaussian process, where its smoothness is dictated
by the choice of kernel function.

\paragraph{Time-varing Gaussian process.}

We first model the time-varying black-box function $f(\bx,t)$ using
GP which is designed to capture the correlation across hyperparameter
$\bx$ and time $t$ as $f(\bx,t)\sim GP\left(0,K([\bx,t],[\bx',t'])\right)$.
To model the correlation across the spatial and temporal spaces, we
can consider the covariance kernel as a product $k\left([\bx,t],[\bx',t']\right)=k(\bx,\bx')\times k_{time}(t,t')$.
Particularly, the covariance function for time is chosen as $k_{time}(t,t')=(1-\omega)^{\frac{|t-t'|}{2}}$
where $\omega$ is a forgetting-remembering trade-off parameter. Larger
$\omega$ indicates that the observations are less correlated and
vice versa.

We consider the noise setting where $y_{i}=f(\bx_{i})+\epsilon_{i}$,
$\epsilon_{i}\sim\mathcal{N}(0,\sigma_{f}^{2})$ and $\sigma_{f}^{2}$
is the noise variance. Under this noise setting, the output follows
the GP as $\by\sim GP(m,\bK+\sigma_{f}^{2}\idenmat)$ that provides
the Gaussian predictive distribution for any point $[\bx_{*},t_{*}]$
with the mean and variance are defined as\vspace{-10pt}

\begin{minipage}[t]{0.48\columnwidth}%
\begin{align}
\mu\left([\bx_{*},t_{*}]\right)= & \mathbf{k}_{*}\left[\mathbf{K}+\sigma_{f}^{2}\idenmat\right]^{-1}\mathbf{y}\label{eq:mu_f}
\end{align}
%
\end{minipage}%
\begin{minipage}[t]{0.48\columnwidth}%
\begin{align}
\sigma^{2}\left([\bx_{*},t_{*}]\right)= & k_{**}-\mathbf{k}_{*}\left[\mathbf{K}+\sigma_{f}^{2}\idenmat\right]^{-1}\mathbf{k}_{*}^{T}\label{eq:sigma_f}
\end{align}
%
\end{minipage}

where $\by=[y_{i}]_{\forall i}$, $\ensuremath{\bk_{*}=[k\left([\bx_{*},t_{*}],[\bx_{i},t_{i}]\right)]_{\forall i}}$,
$\ensuremath{\mathbf{K}=\left[k\left([\bx_{i},t_{i}],[\bx_{j},t_{j}]\right)\right]_{\forall i,j}}$,
$\ensuremath{k_{**}=k\left([\bx_{*},t_{*}],[\bx_{*},t_{*}]\right)}$.
We can learn the kernel hyperparameters of $K$ -- such as length
scale parameter of $k(\bx,\bx')$, $\omega$ of $k_{time}(t,t')$
and noise variance $\sigma_{f}^{2}$ -- by maximizing the log marginal
likelihood \cite{Rasmussen_2006gaussian}.

